On Systematically Building a Controlled Natural Language for Functional Requirements

[Context] Natural language (NL) is pervasive in software requirements specifications (SRSs). However, despite its popularity and widespread use, NL is highly prone to quality issues such as vagueness, ambiguity, and incompleteness. Controlled natural languages (CNLs) have been proposed as a way to prevent quality problems in requirements documents, while maintaining the flexibility to write and communicate requirements in an intuitive and universally understood manner. [Objective] In collaboration with an industrial partner from the financial domain, we systematically develop and evaluate a CNL, named Rimay, intended at helping analysts write functional requirements. [Method] We rely on Grounded Theory for building Rimay and follow well-known guidelines for conducting and reporting industrial case study research. [Results] Our main contributions are: (1) a qualitative methodology to systematically define a CNL for functional requirements; this methodology is general and applicable to information systems beyond the financial domain, (2) a CNL grammar to represent functional requirements; this grammar is derived from our experience in the financial domain, but should be applicable, possibly with adaptations, to other information-system domains, and (3) an empirical evaluation of our CNL (Rimay) through an industrial case study. Our contributions draw on 15 representative SRSs, collectively containing 3215 NL requirements statements from the financial domain. [Conclusion] Our evaluation shows that Rimay is expressive enough to capture, on average, 88% (405 out of 460) of the NL requirements statements in four previously unseen SRSs from the financial domain.

==> ExternalValidity.tex <==
%!TEX root = main.tex
%\subsection{External validity}
%External validity is concerned with the extent to which it is possible to generalize the findings, and to what extent the findings are of interest to other people outside the investigated case \cite{Runeson:2012}. 

%Since in this study, we built our CNL by relying on representative SDRs provided by our Clearstream, it is natural to assume that our CNL grammar rules may be specific to the financial domain. To mitigate this limitation, we used domain-independent lexical resources such as VerbNet and WordNet and we did not include in our CNL any keyword specific to the financial domain. By doing so, we hope that our CNL can at least serve as a strong basis to address the needs of other application domains. 
%Lionel: Our research question, as currently stated, never implied we wanted to serve the needs of other domains. So, in this case, this is not a threat. But we should clarify earlier that, beyond the financial domain, our ambition is to develop a CNL that widely addresses the needs in information systems. Also, the reader might even question whether the selected SRDs are representative of the financial domain. We never argued earlier why they were. 

%In our case, the threat to external validity is whether the conclusion can be generalized to other functional NLRs written by other companies and other domains. We believe that our findings can be generalized to other companies in the financial domain because we do not include keywords in our CNL that correspond to concepts invented or used exclusively by our industrial partner. Furthermore, our CNL can be generalized to similar domains, such as information systems, because we avoided the introduction of jargon used by the analysts, and we used a domain-independent lexicon to construct our grammar rules. The objective of the validation of our CNL was of exploratory nature, where we wanted to reveal  qualitative and quantitative insights about our CNL and how it was created. Needed are, therefore, further independent investigations were it has to be examined how our CNL is further specialized to  other companies.

==> listings/GeneralGrammar_A.tex <==
REQUIREMENT: SCOPE? CONDITION_STRUCTURES? ARTICLE? ACTOR MODAL_VERB not?  SYSTEM_RESPONSE.
CONDITION_STRUCTURES: CONDITION_STRUCTURE (,? (and|or) CONDITION_STRUCTURE)*, then?
SCOPE: For MODIFIER? TEXT (and MODIFIER? TEXT)?,
CONDITION_STRUCTURE: WHILE_STRUCTURE|WHEN_STRUCTURE|WHERE_STRUCTURE|IF_STRUCTURE|TEMPORAL_STRUCTURE
WHILE_STRUCTURE: While PRECONDITION_STRUCTURE
WHEN_STRUCTURE: When TRIGGER
WHERE_STRUCTURE: Where TEXT #TEXT is a feature expression
IF_STRUCTURE: If PRECONDITION_STRUCTURE|TRIGGER
TEMPORAL_STRUCTURE: (Before|After)(TIME|TRIGGER)

WHEN_STRUCTURE: When (TRIGGER|TEXT)
IF_STRUCTURE: If (PRECONDITION_STRUCTURE|TRIGGER)
WHERE_STRUCTURE: Where TEXT #TEXT must describe features of the system

==> listings/GeneralGrammar_B.tex <==
TRIGGER: MODIFIER? ACTOR ACTIONS_EXPRESSION
ACTION: ((do|does) not )? ACTION_PHRASE
PRECONDITION_STRUCTURE: ITEMIZED_CONDITIONS | CONDITIONS_EXPRESSION 
TIME: TEXT UNIT #TEXT describes an amount of time units
ITEMIZED_CONDITIONS: the following conditions are satisfied:
	HYPHEN CONDITION((,|,and|and) 
	HYPHEN CONDITION)+


ACTIONS_IN_TRIGGER: ((do|does) not )? ACTION_PHRASE | UI_ACTION)
UI_ACTION: (TEXT | (right|left|double) )? #e.g., right click, double clicks
	clicks|focuses|ticks|opens
	(TEXT | twice)?#e.g., click 'twice'
	on?
	MODIFIER?
	UIComponentInstance

==> listings/GeneralGrammar_C.tex <==
CONDITION: INSTANCE_OR_CLASS_HAS_PROPERTIES | CONVENTION | ACTOR_OR_CLASS_OR_PROPERTY_OPERATOR_ELEMENT | INSTANCE_OR_PROPERTY_OPERATOR_VALUE | UI_COMPONENT_INSTANCE_OPERATOR_ELEMENT | TEXT 

INSTANCE_OR_CLASS_HAS_PROPERTIES: MODIFIER? (INSTANCE|CLASS) CONTAINS (the properties described in TEXT)|(the (property|properties): PROPERTIES)

CONVENTION: ((TEXT (of CLASS)? | PROPERTY) (conforms|conform|comply|complies) (to|with) MODIFIER? (format|convention|standard) TEXT 

CLASS_OR_PROPERTY_OPERATOR_VALUE: MODIFIER? CLASS|PROPERTY OPERATOR_VALUES_EXPR

INSTANCE_OR_PROPERTY_OPERATOR_VALUE:	MODIFIER? TEXT OF_CLASS_OR_REFERENCE_TO_LABEL? Label? OPERATOR_VALUES_EXPR

UI_COMPONENT_INSTANCE_OPERATOR_ELEMENT: MODIFIER? TEXT UI_COMPONENT OPERATOR_VALUES_EXPR

OPERATOR_VALUES_EXPR: (COMPARE|CONTAINS|OTHER_OPERATORS) MODIFIER? MULTI_VALUES_EXPR TEXT?





///
CONDITION: INSTANCE_HAS_PROPERTIES | CONVENTION | ACTOR_OR_TYPE_OR_PROPERTY_OPERATOR_ELEMENT | INSTANCE_OR_PROPERTY_OPERATOR_VALUE | UI_COMPONENT_INSTANCE_OPERATOR_ELEMENT | TEXT 

INSTANCE_HAS_PROPERTIES: MODIFIER? NON_UI_COMPONENT_INSTANCE 
	CONTAINS ((the properties described in TEXT)|(the (property|properties): TEXT))

CONVENTION: ((TEXT (of [TYPE_OR_LABEL|ID])? | [PROPERTY|ID_DOT_ID]) 
  (conforms|conform|comply|complies) (to|with) MODIFIER? (format|convention|standard) TEXT 

TYPE_OR_PROPERTY_OPERATOR_VALUE: MODIFIER? [TYPE_OR_PROPERTY|ID_DOT_ID] OPERATOR_VALUES_EXPR

INSTANCE_OR_PROPERTY_OPERATOR_VALUE:	MODIFIER? TEXT OF_TYPE_OR_REFERENCE_TO_LABEL? Label? OPERATOR_VALUES_EXPR

UI_COMPONENT_INSTANCE_OPERATOR_ELEMENT: MODIFIER? TEXT [UI_COMPONENT] OPERATOR_VALUES_EXPR

OPERATOR_VALUES_EXPR: (COMPARE | CONTAINS | OTHER_OPERATORS) MODIFIER? MULTI_VALUES_EXPR TEXT?

==> listings/GeneralGrammar_D.tex <==
SYSTEM_RESPONSE: SYSTEM_RESPONSE_EXPRESSION | RESPONSE_BLOCK_ITEMIZED
ATOMIC_SYSTEM_RESPONSE: ACTION_PHRASE (every TEXT )?
RESPONSE_BLOCK_ITEMIZED: do the following actions (in sequence)? : 
	BULLET ATOMIC_SYSTEM_RESPONSE ((,|, and|, or|and|or)? 
	BULLET ATOMIC_SYSTEM_RESPONSE) *
		
		
SYSTEM_RESPONSE: ARTICLE? [ACTOR] MODAL_VERB RESPONSE_BLOCK
RESPONSE_BLOCK: SYSTEM_RESPONSE_EXPRESSION | RESPONSE_BLOCK_ITEMIZED
ATOMIC_SYSTEM_RESPONSE: MODAL_VERB? not? ACTION_PHRASE (every TEXT )?
RESPONSE_BLOCK_ITEMIZED: do the following actions (in sequence)? : 
	BULLET ATOMIC_SYSTEM_RESPONSE ((,|, and|, or|and|or)? 
	BULLET ATOMIC_SYSTEM_RESPONSE) *

==> ref_old.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Mauricio ALFEREZ at 2019-06-12 13:34:31 +0200


%% Saved with string encoding Unicode (UTF-8)

@book{GlaStr67,
  added-at = {2010-01-29T10:11:35.000+0100},
  address = {New York, NY},
  author = {Glaser, Barney G. and Strauss, Anselm L.},
  publisher = {Aldine de Gruyter},
  title = {The Discovery of Grounded Theory: Strategies for Qualitative Research},
  year = 1967
}

@article{Badampudi2016,
title = "Software component decision-making: In-house, OSS, COTS or outsourcing - A systematic literature review",
journal = "Journal of Systems and Software",
volume = "121",
pages = "105 - 124",
year = "2016",
issn = "0164-1212",
doi = "https://doi.org/10.1016/j.jss.2016.07.027",
url = "http://www.sciencedirect.com/science/article/pii/S0164121216301212",
author = "Deepika Badampudi and Claes Wohlin and Kai Petersen",
keywords = "OSS, COTS, In-house development, Outsourcing, Decision-making, Component-based software engineering",
}

@book{bettini2016implementing,
  title={Implementing domain-specific languages with Xtext and Xtend},
  author={Bettini, Lorenzo},
  year={2016},
  publisher={Packt Publishing Ltd}
}

@article{rupp2009requirements,
  title={Requirements engineering und management},
  author={Rupp, Chris and Simon, Matthias and Hocker, Florian},
  journal={HMD Praxis der Wirtschaftsinformatik},
  volume={46},
  number={3},
  pages={94--103},
  year={2009},
  publisher={Springer}
}

@book{Runeson:2012,
 author = {Runeson, Per and Host, Martin and Rainer, Austen and Regnell, Bjorn},
 title = {Case Study Research in Software Engineering: Guidelines and Examples},
 year = {2012},
 isbn = {1118104358, 9781118104354},
 edition = {1st},
 publisher = {Wiley Publishing},
}

@article{Luisa:2004,
 author = {Luisa, Mich and Mariangela, Franch and Pierluigi, Inverardi},
 title = {Market Research for Requirements Analysis Using Linguistic Tools},
 journal = {Requir. Eng.},
 issue_date = {February 2004},
 volume = {9},
 number = {1},
 month = feb,
 year = {2004},
 issn = {0947-3602},
 pages = {40--56},
 numpages = {17},
 url = {http://dx.doi.org/10.1007/s00766-003-0179-8},
 doi = {10.1007/s00766-003-0179-8},
 acmid = {1008824},
 publisher = {Springer-Verlag New York, Inc.},
 address = {Secaucus, NJ, USA},
 keywords = {Conceptual modelling, Market research, NLP-based CASE tools, Potential demand, Requirements analysis},
}

@ARTICLE{Boehm:2001,
author={B. {Boehm} and V. R. {Basili}},
journal={Computer},
title={Top 10 list [software development]},
year={2001},
volume={34},
number={1},
pages={135-137},
doi={10.1109/2.962984},
ISSN={},
month={Jan},}

@book{Dick2017,
  title={Requirements Engineering},
  author={Jeremy Dick and Elizabeth Hull and Ken Jackson},
  year={2017},
 publisher = {Springer International Publishing},
}

@Article{Young:2015,
author="Young, R.",
title="The Main Thing is Keeping the Main Thing the Main Thing",
journal="Requirements Engineering Magazine ",
year="2015",
volume="1"
}
@inproceedings{solemon2009requirements,
  title={Requirements engineering problems and practices in software companies: An industrial survey},
  author={Solemon, Badariah and Sahibuddin, Shamsul and Ghani, Abdul Azim Abd},
  booktitle={International conference on advanced software engineering and its applications},
  pages={70--77},
  year={2009},
  organization={Springer}
}

@Article{Sadraei:2007,
author="Sadraei, Emila
and Aurum, Ayb{\"u}ke
and Beydoun, Ghassan
and Paech, Barbara",
title="A field study of the requirements engineering practice in Australian software industry",
journal="Requirements Engineering",
year="2007",
month="Jul",
day="01",
volume="12",
number="3",
pages="145--162",
issn="1432-010X",
doi="10.1007/s00766-007-0042-4",
url="https://doi.org/10.1007/s00766-007-0042-4"
}

@misc{ UML25,
    author = "{OMG}",
    title = "Unified Modeling Language. Version 2.5",
    year = "2015",
    Institution = {Object Management Group, Inc},
    url = "http://www.omg.org/spec/UML/2.5/",
    note = "Accessed 27 February 2020"
  }


@book{Robson:2016,
 author = {Robson, Colin and McCartan, Kieran},
 title = {Real World Research},
 year = {2016},
 isbn = {978-1-118-74523-6},
 edition = {4th},
 publisher = {Wiley Publishing},
}

@Article{Lethbridge2005,
author="Lethbridge, Timothy C.
and Sim, Susan Elliott
and Singer, Janice",
title="Studying Software Engineers: Data Collection Techniques for Software Field Studies",
journal="Empirical Software Engineering",
year="2005",
month="Jul",
day="01",
volume="10",
number="3",
pages="311--341",
}

@book{Wohlin:2012,
 author = {Wohlin, Claes and Runeson, Per and Hst, Martin and Ohlsson, Magnus C. and Regnell, Bjrn and Wessln, Anders},
 title = {Experimentation in Software Engineering},
 year = {2012},
 isbn = {3642290434, 9783642290435},
 publisher = {Springer Publishing Company, Incorporated},
}

@misc{clearstreamWeb,
Author = {{Clearstream}},
Howpublished = {https://www.clearstream.com},
Owner = {alferez},
Timestamp = {2019.08.07},
year = {2020},
Title = {Clearstream services {SA}}}

@inproceedings{AlferezModels19,
  author    = {Mauricio Alf{\'{e}}rez and
               Fabrizio Pastore and
               Mehrdad Sabetzadeh and
               Lionel C. Briand and
               Jean{-}Richard Riccardi},
  editor    = {Marouane Kessentini and
               Tao Yue and
               Alexander Pretschner and
               Sebastian Voss and
               Loli Burgue{\~{n}}o},
  title     = {Bridging the Gap between Requirements Modeling and Behavior-Driven
               Development},
  booktitle = {22nd {ACM/IEEE} International Conference on Model Driven Engineering
               Languages and Systems, {MODELS} 2019, Munich, Germany, September 15-20,
               2019},
  pages     = {239--249},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/MODELS.2019.00008},
  doi       = {10.1109/MODELS.2019.00008},
  timestamp = {Mon, 02 Dec 2019 08:27:36 +0100},
  biburl    = {https://dblp.org/rec/conf/models/AlferezPSBR19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{EA,
	Author = {{SPARX}},
	Howpublished = {https://sparxsystems.com/products/ea/},
	Owner = {pastore},
	year={2020},
	Timestamp = {2014.08.13},
	Title = {Enterprise Architect}}

@book{crystal2011dictionary,
  title={A Dictionary of Linguistics and Phonetics},
  author={Crystal, D.},
  isbn={9781444356755},
  series={The Language Library},
  year={2011},
  publisher={Wiley}
}
@book{saldana2015coding,
  title={The coding manual for qualitative researchers},
  author={Salda{\~n}a, Johnny},
  year={2015},
  publisher={Sage}
}
@book{auerbach2003qualitative,
  title={Qualitative data: An introduction to coding and analysis},
  author={Auerbach, Carl and Silverstein, Louise B},
  year={2003},
  publisher={NYU press}
}

@misc{WordNet,
	Author = {{Princeton University}},
	Date-Added = {2019-06-07 16:34:47 +0200},
	Date-Modified = {2019-06-07 16:35:29 +0200},
	Howpublished = {https://wordnet.princeton.edu/},
	Title = {{About WordNet"}},
	Year = {2020}}

@misc{Xtext,
	Author = {{Eclipse Foundation}},
	Date-Added = {2019-06-05 11:35:45 +0200},
	Date-Modified = {2019-06-06 09:02:33 +0200},
	Howpublished = {https://www.eclipse.org/Xtext/},
	Title = {Xtext},
	Year = {2020},
	Bdsk-Url-1 = {https://www.eclipse.org/Xtext/}}

@misc{ApachePOI,
	Author = {{Apache Software Foundation}},
	Date-Added = {2019-06-05 11:33:25 +0200},
	Date-Modified = {2019-06-06 09:02:52 +0200},
	Howpublished = {https://poi.apache.org/},
	Title = {Apache {POI}},
	Year = {2020},
	Bdsk-Url-1 = {https://poi.apache.org/}}

@inproceedings{Falkner:19,
	Author = {Falkner, Andreas and Palomares, Cristina and Franch, Xavier and Schenner, Gottfried and Aznar, Pablo and Schoerghuber, Alexander},
	Booktitle = {Proceedings of the 25th International Working Conference on Requirements Engineering: Foundation for Software Quality (REFSQ'19)},
	Date-Modified = {2019-03-30 20:57:45 +0000},
	Pages = {176--182},
	Title = {Identifying Requirements in Requests for Proposal: A Research Preview},
	Year = {2019}}

@inproceedings{Winkler:16,
	Author = {J. Winkler and A. Vogelsang},
	Booktitle = {Proceedings of the 24th International Requirements Engineering Conference Workshops (REW'16)},
	Date-Modified = {2019-03-30 20:30:48 +0000},
	Pages = {39-45},
	Title = {Automatic Classification of Requirements Based on Convolutional Neural Networks},
	Year = {2016}}

@inproceedings{mavin2009easy,
  title={Easy approach to requirements syntax (EARS)},
  author={Mavin, Alistair and Wilkinson, Philip and Harwood, Adrian and Novak, Mark},
  booktitle={2009 17th IEEE International Requirements Engineering Conference},
  pages={317--322},
  year={2009},
  organization={IEEE}
}

@inproceedings{DBLP:conf/re/MavinWGU16,
	Author = {Alistair Mavin and Philip Wilkinson and Sarah Gregory and Eero Uusitalo},
	Booktitle = {{RE}},
	Pages = {276--282},
	Publisher = {{IEEE} Computer Society},
	Title = {Listens Learned {(8} Lessons Learned Applying {EARS)}},
	Year = {2016}}

@article{ahonen2010software,
	Author = {Ahonen, Jarmo J and Savolainen, Paula},
	Journal = {Journal of Systems and Software},
	Number = {11},
	Pages = {2175--2187},
	Publisher = {Elsevier},
	Title = {Software engineering projects may fail before they are started: Post-mortem analysis of five cancelled projects},
	Volume = {83},
	Year = {2010}}

@misc{elizabeth2011requirements,
	Author = {Elizabeth, Hull and Jackson, K and Dick, Jeremy},
	Publisher = {Springer},
	Title = {Requirements engineering},
	Year = {2011}}


@article{rupp2004requirements,
  title={Requirements Templates --The Blueprint of your Requirement},
  author={Rupp, Christine},
  journal={Requirement Engineering},
  year={2004}
}

@inproceedings{eckhardt2016challenging,
	Author = {Eckhardt, Jonas and Vogelsang, Andreas and Femmer, Henning and Mager, Philipp},
	Booktitle = {2016 IEEE 24th International Requirements Engineering Conference (RE)},
	Organization = {IEEE},
	Pages = {46--55},
	Title = {Challenging incompleteness of performance requirements by sentence patterns},
	Year = {2016}}

@book{withall2007software,
	Author = {Withall, Stephen},
	Publisher = {Pearson Education},
	Title = {Software requirement patterns},
	Year = {2007}}

@book{PohlKlaus2010Re:f,
  author    = {Klaus Pohl},
  title     = {Requirements Engineering - Fundamentals, Principles, and Techniques},
  publisher = {Springer},
  year      = {2010},
  isbn      = {978-3-642-12577-5},
  timestamp = {Fri, 04 Feb 2011 11:23:26 +0100},
  biburl    = {https://dblp.org/rec/books/daglib/0024869.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{arora2015automated,
	Author = {Arora, Chetan and Sabetzadeh, Mehrdad and Briand, Lionel and Zimmer, Frank},
	Journal = {IEEE transactions on Software Engineering},
	Number = {10},
	Pages = {944--968},
	Publisher = {IEEE},
	Title = {Automated checking of conformance to requirements templates using natural language processing},
	Volume = {41},
	Year = {2015}}

@inproceedings{moitra2018towards,
	Author = {Moitra, Abha and Siu, Kit and Crapo, Andrew and Chamarthi, Harsh and Durling, Michael and Li, Meng and Yu, Han and Manolios, Panagiotis and Meiners, Michael},
	Booktitle = {2018 IEEE 26th International Requirements Engineering Conference (RE)},
	Organization = {IEEE},
	Pages = {286--296},
	Title = {Towards Development of Complete and Conflict-Free Requirements},
	Year = {2018}}

@inproceedings{post2011applying,
	Author = {Post, Amalinda and Menzel, Igor and Podelski, Andreas},
	Booktitle = {International Working Conference on Requirements Engineering: Foundation for Software Quality},
	Organization = {Springer},
	Pages = {166--180},
	Title = {Applying Restricted English Grammar onAutomotive Requirements -- Does it Work? A Case Study},
	Year = {2011}}

@incollection{fuchs2008attempto,
	Author = {Fuchs, Norbert E and Kaljurand, Kaarel and Kuhn, Tobias},
	Booktitle = {Reasoning Web},
	Pages = {104--124},
	Publisher = {Springer},
	Title = {Attempto controlled english for knowledge representation},
	Year = {2008}}

@inproceedings{konrad2005real,
	Author = {Konrad, Sascha and Cheng, Betty HC},
	Booktitle = {Proceedings of the 27th international conference on Software engineering},
	Organization = {ACM},
	Pages = {372--381},
	Title = {Real-time specification patterns},
	Year = {2005}}

@inproceedings{bernth1997easyenglish,
	Author = {Bernth, Arendse},
	Booktitle = {Proceedings of the fifth conference on Applied natural language processing},
	Organization = {Association for Computational Linguistics},
	Pages = {159--165},
	Title = {EasyEnglish: a tool for improving document quality},
	Year = {1997}}

@inproceedings{kamprath1998controlled,
  title={Controlled language for multilingual document production: Experience with Caterpillar technical English},
  author={Kamprath, Christine and Adolphson, Eric and Mitamura, Teruko and Nyberg, Eric},
  booktitle={Proceedings of the Second International Workshop on Controlled Language Applications},
  volume={146},
  year={1998}
}

@book{BrinkBook,
	Address = {Greenwich, CT, USA},
	Author = {Brink, Henrik and Richards, Joseph and Fetherolf, Mark},
	Edition = {1st},
	Isbn = {1617291927, 9781617291920},
	Publisher = {Manning Publications Co.},
	Title = {Real-World Machine Learning},
	Year = {2016}}

@inproceedings{filipovikj2014reassessing,
  title={Reassessing the pattern-based approach for formalizing requirements in the automotive domain},
  author={Filipovikj, Predrag and Nyberg, Mattias and Rodriguez-Navas, Guillermo},
  booktitle={2014 IEEE 22nd International Requirements Engineering Conference (RE)},
  pages={444--450},
  year={2014},
  organization={IEEE}
}

@article{miller1995wordnet,
  title={WordNet: a lexical database for English},
  author={Miller, George A},
  journal={Communications of the ACM},
  volume={38},
  number={11},
  pages={39--41},
  year={1995},
  publisher={ACM}
}


@inproceedings{kipper2000verbnet,
  author    = {Karin Kipper and
               Hoa Trang Dang and
               Martha Stone Palmer},
  editor    = {Henry A. Kautz and
               Bruce W. Porter},
  title     = {Class-Based Construction of a Verb Lexicon},
  booktitle = {Proceedings of the Seventeenth National Conference on Artificial Intelligence
               and Twelfth Conference on on Innovative Applications of Artificial
               Intelligence, July 30 - August 3, 2000, Austin, Texas, {USA}},
  pages     = {691--696},
  publisher = {{AAAI} Press / The {MIT} Press},
  year      = {2000},
  url       = {http://www.aaai.org/Library/AAAI/2000/aaai00-106.php},
  timestamp = {Tue, 11 Dec 2012 12:57:22 +0100},
  biburl    = {https://dblp.org/rec/conf/aaai/KipperDP00.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{crapo2017requirements,
  title={Requirements capture and analysis in ASSERT (TM)},
  author={Crapo, Andrew and Moitra, Abha and McMillan, Craig and Russell, Daniel},
  booktitle={2017 IEEE 25th International Requirements Engineering Conference (RE)},
  pages={283--291},
  year={2017},
  organization={IEEE}
}
@article{kopczynska2018empirical,
  title={An empirical study on catalog of non-functional requirement templates: Usefulness and maintenance issues},
  author={Kopczy{\'n}ska, Sylwia and Nawrocki, Jerzy and Ochodek, Miros{\l}aw},
  journal={Information and Software Technology},
  volume={103},
  pages={75--91},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{riaz2014hidden,
  author    = {Maria Riaz and
               Jason Tyler King and
               John Slankas and
               Laurie A. Williams},
  editor    = {Tony Gorschek and
               Robyn R. Lutz},
  title     = {Hidden in plain sight: Automatically identifying security requirements
               from natural language artifacts},
  booktitle = {{IEEE} 22nd International Requirements Engineering Conference, {RE}
               2014, Karlskrona, Sweden, August 25-29, 2014},
  pages     = {183--192},
  publisher = {{IEEE} Computer Society},
  year      = {2014},
  url       = {https://doi.org/10.1109/RE.2014.6912260},
  doi       = {10.1109/RE.2014.6912260},
  timestamp = {Wed, 16 Oct 2019 14:14:56 +0200},
  biburl    = {https://dblp.org/rec/conf/re/RiazKSW14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{mavin2010big,
  title={Big ears (the return of" easy approach to requirements engineering")},
  author={Mavin, Alistair and Wilkinson, Philip},
  booktitle={2010 18th IEEE International Requirements Engineering Conference},
  pages={277--282},
  year={2010},
  organization={IEEE}
}
@article{carvalho2014nat2testscr,
  title={NAT2TESTSCR: Test case generation from natural language requirements based on SCR specifications},
  author={Carvalho, Gustavo and Falc{\~a}o, Diogo and Barros, Fl{\'a}via and Sampaio, Augusto and Mota, Alexandre and Motta, Leonardo and Blackburn, Mark},
  journal={Science of Computer Programming},
  volume={95},
  pages={275--297},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{denger2003higher,
  title={Higher quality requirements specifications through natural language patterns},
  author={Denger, Christian and Berry, Daniel M and Kamsties, Erik},
  booktitle={Proceedings 2003 Symposium on Security and Privacy},
  pages={80--90},
  year={2003},
  organization={IEEE}
}

@misc{ChaosReport,
  author = {{The Standish Group}},
  publisher = {{The Standish Group}},
  title = {The Chaos Report},
  year = {1995-2019}
}

@inproceedings{DBLP:conf/ecmdafa/YueAB11,
  author    = {Tao Yue and
               Shaukat Ali and
               Lionel C. Briand},
  title     = {Automated Transition from Use Cases to {UML} State Machines to Support
               State-Based Testing},
  booktitle = {{ECMFA}},
  series    = {Lecture Notes in Computer Science},
  volume    = {6698},
  pages     = {115--131},
  publisher = {Springer},
  year      = {2011}
}

@article{yue2011systematic,
  title={A systematic review of transformation approaches between user requirements and analysis models},
  author={Yue, Tao and Briand, Lionel C and Labiche, Yvan},
  journal={Requirements engineering},
  volume={16},
  number={2},
  pages={75--99},
  year={2011},
  publisher={Springer}
}

@ARTICLE{arora2017automated,  
    author={C. {Arora} and M. {Sabetzadeh} and L. {Briand} and F. {Zimmer}},          journal={IEEE Transactions on Software Engineering},     
    title={Automated Extraction and Clustering of Requirements Glossary Terms},   
    year={2017},             
    volume={43},  
    number={10},  
    pages={918-945},
}

@book{pohl_rupp_2011,
  author    = {Klaus Pohl and
               Chris Rupp},
  title     = {Requirements Engineering Fundamentals - {A} Study Guide for the Certified
               Professional for Requirements Engineering Exam: Foundation Level -
               {IREB} compliant},
  publisher = {Rocky Nook},
  year      = {2011},
  isbn      = {978-1-933952-81-9},
  timestamp = {Wed, 04 Mar 2015 17:02:57 +0100},
  biburl    = {https://dblp.org/rec/books/daglib/0034874.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{Dietterich98,
  author    = {Thomas G. Dietterich},
  title     = {Approximate Statistical Test For Comparing Supervised Classification
               Learning Algorithms},
  journal   = {Neural Computation},
  volume    = {10},
  number    = {7},
  pages     = {1895--1923},
  year      = {1998},
  url       = {https://doi.org/10.1162/089976698300017197},
  doi       = {10.1162/089976698300017197},
  timestamp = {Wed, 14 Nov 2018 10:31:17 +0100},
  biburl    = {https://dblp.org/rec/journals/neco/Dietterich98.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
